Multi-Level Correlation Network For Few-Shot Image Classification

Few-shot image classification(FSIC) aims to recognize novel classes given few labeled images from base classes. Recent works have achieved promising classification performance, especially for metric-learning methods, where a measure at only image feature level is usually used. In this paper, we argue that measure at such a level may not be effective enough to generalize from base to novel classes when using only a few images. Instead, a multi-level descriptor of an image is taken for consideration in this paper. We propose a multi-level correlation network (MLCN) for FSIC to tackle this problem by effectively capturing local information. Concretely, we present the self-correlation module and cross-correlation module to learn the semantic correspondence relation of local information based on learned representations. Moreover, we propose a pattern-correlation module to capture the pattern of fine-grained images and find relevant structural patterns between base classes and novel classes. Extensive experiments and analysis show the effectiveness of our proposed method on four widely-used FSIC benchmarks. The code for our approach is available at: https://github.com/Yunkai696/MLCN.

==> tables/compare.tex <==
	\begin{table}[t]
	\centering%
	\resizebox{1.0\columnwidth}{!}{
	\begin{tabular}{lcccccccc}
					\toprule
					Method & Type & global & local & \thead{CUB \\ 5way5shot} &  \\
					\midrule
                    ProNet~\cite{protonet} &  One-stage & $\times$ &  \Checkmark &  82.50 ± 0.58  \\
					MAML~\cite{finn2017model} &  One-stage & $\times$ &  \Checkmark &  83.47 ± 0.59  \\
                    CloserLook~\cite{closer} &  One-stage & \Checkmark &  $\times$ & 64.16 ± 0.71    \\
                    CloserLook++~\cite{} &  One-stage & \Checkmark &  $\times$ & 79.34 ± 0.61    \\
					DeepEMD~\cite{deepemd} &  two-stage  & \Checkmark &  \Checkmark & 88.69 ± 0.50    \\
                    BML~\cite{BML} &  One-stage & \Checkmark &  \Checkmark   & 90.45 ± 0.36   \\
					\midrule
					\textbf{Ours} &  One-stage & \Checkmark & \Checkmark&\textbf{91.20 ± 0.24 }  \\ % long scale
					\bottomrule
			\end{tabular}}
		\label{table:compare}
        \caption{ Accuracy $\left (  \% \right ) $ and the number of additional learnable pa-rameters of other relation-based methods.and un-derline denotes the best performance among others.}%\vspace{-1mm}
	\end{table}



==> tables/comparision.tex <==
\begin{table*}[htbp]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}[b]{lccccr}
   \toprule
    method & CUB-200-2011  & 5-way  & 5-way 5-shot\\  \midrule
    \emph{cosine} classifier~\cite{closer} & \emph{ResNet12}  & 55.43 $\pm$ 0.81 & 77.18 $\pm$ 0.61 \\
    TADAM~\cite{tadam}  & \emph{ResNet12}  & 58.50 $\pm$ 0.30 & 76.70 $\pm$ 0.30 \\
    Shot-Free~\cite{shotfree}  & \emph{ResNet12}  & 59.04   & 77.64   \\
    TPN~\cite{tpn}  & \emph{ResNet12}  & 59.46   & 75.65  \\
    PPA~\cite{qiao2018few}  & \emph{WRN\small{-28-10}}${}^{\dag}$  & 59.60 $\pm$ 0.41  & 73.74  $\pm$ 0.19 \\
    FEAT~\cite{feat}  & \emph{ResNet12}  & 66.78 $\pm$ 0.20 & 82.05 $\pm$ 0.14\\\midrule
    \textbf{baseline }  & \emph{ResNet12}  & \textbf{67.60 $\pm$ 0.44} & \textbf{82.58 $\pm$ 0.30} \\
    \textbf{\ours (ours-cross)}  & \emph{ResNet12}  & \textbf{67.60 $\pm$ 0.44} & \textbf{82.58 $\pm$ 0.30} \\
    \textbf{\ours (ours-local)}  & \emph{ResNet12}  & \textbf{67.60 $\pm$ 0.44} & \textbf{82.58 $\pm$ 0.30} \\
    \textbf{\ours (local+cross)}  & \emph{ResNet12}  & \textbf{67.60 $\pm$ 0.44} & \textbf{82.58 $\pm$ 0.30} 
    \\\bottomrule 
    \end{tabular}
    }
    \caption{
    Accuracy (\%) and the number of additional learnable parameters of other relation-based methods. 
    ``*'' denotes reproduced one under a controlled environment for a fair comparison, and underline denotes the best performance among others.
    }
\vspace{-5mm}
\end{table*}


==> tables/other_table.tex <==
\begin{table}{t!}
\scalebox{0.95}{
\caption{\small Results on CIFAR-FS dataset.}
\label{table_Cifar}
\begin{tabular}{lccc}
    \toprule
    Mthod & Backbone & 5-way 1-shot & 5-way 5-shot\\  
    \midrule
    R2D2~\cite{bertinetto2018meta}  & \emph{ResNet12}  & 65.30 $\pm$ 0.02 & 78.30 $\pm$ 0.02\\
    \midrule
    RelationNet\cite{RelationNet} & \emph{ResNet12}  &55.50 $\pm$1.00  & 69.30 $\pm$ 0.80\\
    CC~\cite{closer} & \emph{ResNet12}  & 60.39 $\pm$ 0.28 & 72.85 $\pm$ 0.65 \\ %
    Shot-Free~\cite{shotfree} & \emph{ResNet12}  & 69.2 $\pm$ 0.8 & 84.7$\pm$ 0.80 \\
    RFS-simple~\cite{rfs}  & \emph{ResNet12} & 71.5 $\pm$ 0.80  & 86.0 $\pm$ 0.50 \\
    %S2M2~\cite{s2m2} & \emph{ResNet34}${}^{\dag}$  & 62.77 $\pm$ 0.23 & 75.75 $\pm$ 0.13 \\
    ProtoNet~\cite{protonet} & \emph{ResNet12}  & 72.2 $\pm$ 0.70  & 83.5 $\pm$ 0.50 \\ %
    MetaOptNet~\cite{metaoptnet} & \emph{ResNet12}  & 72.6 $\pm$ 0.70  & 84.3 $\pm$ 0.50\\
    %DeepEMD\cite{deepemd} & \emph{ResNet12}  &46.47 $\pm$0.70  & 63.22 $\pm$ 0.71\\
    %MAML\cite{finn2017model} & \emph{ConvNet}  &58.90 $\pm$1.90  & 71.50 $\pm$ 1.00\\
    \midrule
    \textbf{(Ours)}  & \emph{ResNet12} & \textbf{74.36 $\pm$ 0.46} & \textbf{87.24 $\pm$ 0.31} \\ 
    \bottomrule 
\end{tabular}
}
\end{table}
